A bending-torsion theory for thin and ultrathin rods as a $\Gamma$-limit of atomistic models

The purpose of this note is to establish two continuum theories for the bending and torsion of inextensible rods as $\Gamma$-limits of 3D atomistic models. In our derivation we study simultaneous limits of vanishing rod thickness $h$ and interatomic distance $\varepsilon$. First, we set up a novel theory for ultrathin rods composed of finitely many atomic fibres ($\varepsilon\sim h$), which incorporates surface energy and new discrete terms in the limiting functional. This can be thought of as a contribution to the mechanical modelling of nanowires. Second, we treat the case where $\varepsilon\ll h$ and recover a nonlinear rod model $-$ the modern version of Kirchhoff's rod theory.

==> resource_macros.tex <==
\makeatletter
\def\@makechapterhead#1{
  {\parindent \z@ \raggedright \normalfont
   \Huge\bfseries \thechapter. #1
   \par\nobreak
   \vskip 20\p@
}}
\def\@makeschapterhead#1{
  {\parindent \z@ \raggedright \normalfont
   \Huge\bfseries #1
   \par\nobreak
   \vskip 20\p@
}}

\makeatother

%To strech matrices:
\makeatletter
\renewcommand*\env@matrix[1][\arraystretch]{%
  \edef\arraystretch{#1}%
  \hskip -\arraycolsep
  \let\@ifnextchar\new@ifnextchar
  \array{*\c@MaxMatrixCols c}}
\makeatother

\makeatletter
\g@addto@macro\bfseries{\boldmath}
\makeatother

%a shortcut
\newcommand{\sst}{\scriptstyle}

% Draw black "slugs" whenever a line overflows, so that we can spot it easily.
\overfullrule=1mm

%%% Macros for definitions, theorems, claims, examples, ... (requires amsthm package)

\theoremstyle{plain}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{claim}[thm]{Claim}
\newtheorem{observ}[thm]{Observation}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{conj}{Conjecture}

\theoremstyle{plain}
\newtheorem{defn}{Definition}[section]

\theoremstyle{remark}
\newtheorem{rem}{Remark}[section]
\newtheorem{example}{Example}[section]

%with this code, one can make e.g. \begin{customlemma}{A.1} with custom numbering 'A.1'
\theoremstyle{plain}
\newtheorem{innercustomgeneric}{\customgenericname}
\providecommand{\customgenericname}{}
\newcommand{\newcustomtheorem}[2]{%
  \newenvironment{#1}[1]
  {%
   \renewcommand\customgenericname{#2}%
   \renewcommand\theinnercustomgeneric{##1}%
   \innercustomgeneric
  }
  {\endinnercustomgeneric}
}
\newcustomtheorem{customthm}{Theorem}
\newcustomtheorem{customlemma}{Lemma}

%%% The field of all real and natural numbers
%\newcommand{\R}{\textup{I}\! \textup{R}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rinf}{\R_{\infty}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}

%%% Transposition of a vector/matrix
\newcommand{\T}[1]{#1^\top}

%%% Various math goodies
\newcommand{\goto}{\rightarrow}
\newcommand{\abs}[1]{\left|{#1}\right|}%abs. hodnota, pouziti: \abs{A}

%%% is equal to by definition
\newcommand\eqdef{\mathrel{\overset{\makebox[0pt]{\mbox{\normalfont\tiny\sffamily def}}}{=}}}

%%% long vertical bar for function restrictions, use it as \restr{f}{A}
\newcommand\restr[2]{{% we make the whole thing an ordinary symbol
  \left.\kern-\nulldelimiterspace % automatically resize the bar with \right
  #1 % the function
  \vphantom{\big|} % pretend it's a little taller at normal size
  \right|_{#2} % this is the delimiter
  }}
  
%%% argmin
\DeclareMathOperator*{\argmin}{\arg\!\min}

\DeclareMathOperator*{\esssup}{ess\,sup\,}

\DeclareMathOperator{\sgn}{sgn}

%%% integral averages (requires the soul pkg)
\newcommand\inta[1]{\text{\st{$\int\limits_{#1}$}}\,}%use as \inta{U}, U under the integral sign
\newcommand\intac[1]{\text{\st{$\int_{#1}$}}}%'compact', domain next to the integral sign
\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\dashint{\Xint-}%an alternative from the web, it should be less buggy for a long integration domain

\def\y{\tilde{y}}
\def\yk{\tilde{y}^{(k)}}
\def\Gkn{G^{(k)}}
\def\bGkn{\bar{G}^{(k)}}
\def\L{\tilde{\Lambda}}
%\def\x{\tilde{x}}
\def\x{x}
\def\Q{\tilde{Q}}
\def\Dkyk{\bar{D}_k\yk}
\def\xc{\x^\circ}%c for 'corner'
\def\zei{\zeta^i}
\newcommand{\tc}[1]{\textcolor{black}{#1}}%teal

\def\zf{z}
%\def\zfb{\breve{\mathfrak{z}}}
\def\zft{\tilde{z}}
\def\zfb{\zft}
\DeclareMathOperator*{\dk2d}{\bar{\nabla}_\mathit{k}^{\rm 2d}}
\DeclareMathOperator*{\d2d}{\bar{\nabla}^{\rm 2d}}
\DeclareMathOperator*{\dgradk}{\bar{\nabla}_\mathit{k}}
\DeclareMathOperator*{\dleft}{\bar{\nabla}_\mathit{k}^{\rm left}}
\DeclareMathOperator*{\dright}{\bar{\nabla}_\mathit{k}^{\rm right}}

%thin films
%\def\yb{\breve{y}}
\def\yb{\y}
\def\ybk{\yb^{(k)}}
\def\Gk{G^{(k)}}
\def\bGk{\bar{G}^{(k)}}
%\def\xb{\breve{x}}
\def\xb{\x}
%\def\Qb{\breve{Q}}
\def\Qb{\Q}
\def\Lkex{\Lambda_k^{\rm ext}}
\def\Lkexc{\Lambda_k'^{,\mathrm{ext}}}
\def\Lkaux{\Lambda_k^{\rm aux}}
\def\Lkauxc{\Lambda_k'^{,\mathrm{aux}}}
\def\Os{\Omega^{\rm ext}}
\def\Lkexb{\tilde{\Lambda}_k^{\rm ext}}
\def\Lkexcb{\tilde{\Lambda}_k'^{,\mathrm{ext}}}
\def\Lkauxb{\tilde{\Lambda}_k^{\rm aux}}
\def\Lkauxcb{\tilde{\Lambda}_k'^{,\mathrm{aux}}}

%operátory
\renewcommand{\det}{{\rm det}\, }
\newcommand{\cof}{{\rm cof}\, }
\newcommand{\md}{\textup{d}}
\newcommand{\e}{\varepsilon}
\newcommand{\wto}{\rightharpoonup}
\renewcommand{\a}{\alpha}
\renewcommand{\b}{\beta}
\newcommand{\s}{\sigma}
\newcommand{\g}{\gamma}
\renewcommand{\r}{\varrho}
\newcommand{\A}[1]{\left\langle#1\right\rangle}%angle brackets, use as: \A{y}
\newcommand{\ph}{\varphi}
\renewcommand{\O}{{\Omega}}
\renewcommand{\o}{{\omega}}
\newcommand{\tto}{\buildrel {_{_{_{\mbox{$\hspace*{.5mm}\rightarrow$}}}}}\over{_{\mbox{$\rightarrow$}}}}%stejnom. konvergence

\newcommand{\Id}{\mathrm{Id}}%identita
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calT}{\mathcal{T}}

\newcommand{\aein}{\text{a.e. in}}
\newcommand{\foraa}{\text{for a.a.}}
                          
 \newcommand{\weaksto}{\stackrel{*}{\rightharpoonup}\,}
 \newcommand{\weakto}{{\rightharpoonup}\,}

\newcommand\bbA{\mathbb A}
\newcommand\bbB{\mathbb B}
\newcommand\bbE{\mathbb E}
\newcommand\bbF{\mathbb F}
\newcommand\bbG{\mathbb G}
\newcommand\bbH{\mathbb H}
\newcommand\bbQ{\mathbb Q}
\newcommand\bbR{\mathbb R}
\newcommand\bbZ{\mathbb Z}
\newcommand\pl{\partial}%the 'snail' for a partial derivative
\newcommand{\cb}{\color{blue}}
\newcommand{\cred}{\color{red}}
\newcommand{\cg}{\color{green}} 
\newcommand{\cm}{\color{magenta}}

